Mining Shape Expressions with ShapeIt

We present ShapeIt, a tool for mining specifications of cyber-physical systems (CPS) from their real-valued behaviors. The learned specifications are in the form of linear shape expressions, a declarative formal specification language suitable to express behavioral properties over real-valued signals. A linear shape expression is a regular expression composed of parameterized lines as atomic symbols with symbolic constraints on the line parameters. We present here the architecture of our tool along with the different steps of the specification mining algorithm. We also describe the usage of the tool demonstrating its applicability on several case studies from different application domains.

==> sections/se.tex <==
\section{Shape Expressions}
\label{sec:se}

In this section, we define a variant of shape expressions (SE)~\cite{NickovicQFMD19}, 
which are regular expressions where atomic shapes with unknown parameters play the 
role of atomic primitives. These basic shape primitives are expressions that map 
parameter and signal variables to a parameterized family of idealized signals, such as lines, 
sinusoids, exponentials, etc.  Here we focus on the class of {\em linear} SE that
considers only lines as atomic shapes. In contrast to SE in~\cite{NickovicQFMD19}, 
we also allow {\em conjunction} of atomic shapes to facilitate learning of expressions from 
multi-dimensional data and lift the restriction of discrete-time signals. 
Finally, we choose {\em mean squared error} (MSE) as our measure of noise.

Let $\params = \setof{ \param_{1}, \ldots, \param_{n} }$ be a set of
{\em parameters}. A parameter valuation $\val$ maps
parameters $\param \in \params$ to values $\val(\param) \in \Reals \cup
\{ \bot \}$, where $\bot$ represents the {\em undefined} value.  We
use the shortcut $\val(\params)$ to denote $\setof{ \val(\param_{1}),
\ldots, \val(\param_{n})}$.  A {\em constraint} $\gamma$ over
$\params$ is a Boolean combination of inequalities over $\params$.  We
write $\val \models \gamma$ when the constraint $\gamma$ is satisfied
by the valuation $\val$.  Given $\param \in \params$ and $\param \circ
k$ for $\circ \in \setof{ =, <, \leq, >, \geq }$ and some $k \in \Reals$,
we have that $\val(\param) = \bot$ implies that $\val \not \models
\param \circ k$.  We denote by $\Gamma(\params)$ the set of all
constraints over $\params$.

Let $X$ be a set of signal variables. A {\em signal} $w$ over $X$ is 
a sequence $w = (t_{1}, v_{1})\cdot (t_{2}, v_{2}) \cdots (t_{n}, v_{n})$, 
where $t_{i} \in \mathbb{Q}_{\geq 0}$ is the {\em time-stamp} such that 
for all $1 \leq i < n$, $t_{i} < t_{i+1}$ and $v_{i}$ is a valuation in $V(X)$.
We denote by $|w|=n$ the {\em size} of $w$.  Given two signals 
$w = (t_{1}, v_{1})\cdot (t_{2}, v_{2}) \cdots (t_{n}, v_{n})$ and 
$w' = (t'_{1}, v'_{1})\cdot (t'_{2}, v'_{2}) \cdots (t'_{n}, v'_{n})$, their 
{\em concatenation} $w\cdot w'$ is defined if $t_{n} = t'_{1}$ and 
$v_n = v'_1$ and corresponds to the sequence 
$(t_{1}, v_{1})\cdots (t_{n}, v_{n}) \cdot (t'_{2}, v'_{2}) \cdots (t'_{n}, v'_{n})$. 
Given a signal $w$ of size $n$ and $i,j \in \mathbb{N}$ such that $1 \leq i \leq j \leq n$, 
we denote by $w[i:j]$ the sequence $(t_{i}, v_{i}) \cdots (t_{j}, v_{j})$. 
The \emph{duration} $d$ of a signal is defined as $d = t_n - t_1$. 
We allow signals of null duration $d=0$, which results in the unique signal
with the empty time domain\footnote{The signal with the empty time
domain is equivalent to the empty word in the classical language
theory.}. 
%\cristi{Shall we replace $d=0$ by $t_n - t_1 = 0$? (The duration $d$ has been previously not 
%introduced.) We should probably also refine the definition of a signal with null duration, 
%since a signal with only one data point has also duration $d=0$.}
Let $w = (t_1, v_1) \cdots (t_n, v_n)$ and $\hat{w} = (t_1, \hat{v}_n) \cdots (t_n, \hat{v}_n)$ 
be two signals over $X$ of  size $n$, where $w$ represents the observed signal and
$\hat{w}$ a prediction model. The {\em mean squared error} 
$\MSE(w,\hat{w})$ of $w$ relative to $\hat{w}$ is 
a statistical measure of how well the predictions of a (regression) model
approximates the observations, and is defined as follows:
$$
\MSE(w, \hat{w})  =  \max_{x \in X} \frac{1}{n} \Sigma_{i=1}^{n} (v_i(x) - \hat{v}_i(x))^{2}
$$





\subsection{Shape Expressions}\label{sec:shape-expressions}

We now provide the syntax and semantics of linear SE
defined over the set $X$ of signals and the set $\params$ of parameter
variables.  We define the {\em atomic shape} $\lin_x(a,b,\dvar)$ to be the expression that
maps parameter variables $\{a,b, \dvar \} \subseteq \params$ and the signal
variable $x \in X$ to be a parameterized representation of an idealized line signal, defined as follows:
\begin{eqnarray*}
\lin_x(a,b,\dvar) & \equiv & 
\{w~|~\exists \val. t_{|w|}- t_1 = v(\dvar) \wedge 
\forall i \in [1,|w|], w(x,t_i) = \val(a)t_i + \val(b) \}. 
\label{eq:linshape} 
\end{eqnarray*}


\begin{definition}[Linear SE syntax]
A linear shape expression $\f$ is given by the grammar
\begin{eqnarray*}
\psi & ::= & \lin_x(\xparams) : \gamma \mid \psi_1 \cap \psi_2 \\
\f &::= &\epsilon \mid \psi \mid \f_1 \cup \f_2 \mid \f_1 \cdot \f_2 \mid \f^* \mid \f : \gamma 
\end{eqnarray*}
where $x \in X$, $\xparams \subseteq P$, and $\gamma \in \Gamma(P)$. 
\end{definition}

The symbol $\epsilon$ denotes the {\em empty word}, the operators $\cup$, $\cap$,  $\cdot$ and $*$ denote the classical (extended) regular expression 
{\em union}, {\em intersection}, {\em concatenation} and {\em Kleene star} 
respectively, while $\f : \gamma$ says that $\f$ is {\em constrained} by $\gamma$. We write $\f^i$ as an abbreviation of $\f \cdots \f$ ($i$ times).  
We denote by $\mathbb{L}_X(P)$ the set of expressions of the form $\lin_x(\xparams)$ for $x \in X$ and $\xparams \subseteq P$.
The set of shape expressions over $P$ and $X$ is denoted $\Phi(P,X)$.


The semantics of shape expressions is given as a relation between signals and parameter valuations, which we call a \emph{language}.
We associate with every shape expression  a {\em noisy language} $\L_\nu$ for some noise tolerance threshold $\nu \geq 0$, capturing the $\nu$-approximate meaning of the expression. The {\em exact language} $\L$ capturing the precise meaning of the expression is obtained by setting $\nu$ to zero.
We formally define the noisy language as follows.

\begin{definition}[SE noisy language]%\label{def:se_noisy_lang}
Let $\nu \in \R_{\ge0}$ be a noise tolerance threshold.
The noisy language $\L_\nu$ of a shape expression is defined as follows:
\begin{align*}
\L_\nu(\lin_x(\xparams):\gamma) &= \{ (w,v) \st v(\dvar) = t_{|w|} - t_1, \MSE(w(x), \lin_x(v(\xparams))) \leq \nu \} \\
\L_\nu(\psi_1 \cup \psi_2) &= \L_\nu(\psi_1) \cap \L_\nu(\psi_2) \\
\L_\nu(\epsilon) &= \{ (w,v) \st |w| = 0 \} \\
\L_\nu(\f_1 \cdot \f_2) &= \{(w_1 \cdot w_2, v) \st (w_1,v) \in \L_{\nu}(\f_1) \text{ and } (w_2,v) \in \L_{\nu}(\f_2) \} \\
\L_\nu(\f_1 \cup \f_2) &= \L_\nu(\f_1) \cup \L_\nu(\f_2) \\
\L_\nu(\f^*) &= \bigcup_{i=0}^\infty \L_\nu(\f^i) \\
\L_\nu(\f : \gamma) &= \{ (w,v) \st (w,v) \in \L_\nu(\f) \text{ and } v \models \gamma \}
\end{align*}
% 
\end{definition}


The noisy SE language is defined as the set of all signal/parameter valuation pairs, such that the distance of the signal from the ideal 
shape signal defined by the shape expression and instantiated by the parameter valuation is smaller or equal than the noise threshold.

% \subsection{Shape Automata}\label{sec:shape-automata}

% We now define \emph{shape automata}, which will act as recognizers for shape expressions.
% They are akin to finite state automata in which edges are labeled by shape expressions with 
% unknown parameters, and parameter constraints.
% We will then show that they are inter-translatable to shape expressions.
% \begin{definition}[Shape automata]
% A shape automaton is a tuple $\langle P,X,Q,\Delta,S,F \rangle$, where
% (1) $P$ is the set of \emph{parameters}, (2) $X$ is the set of real-valued \emph{signal variables},
% (3) $Q$ is the set of control \emph{locations}, (4) $\Delta \subseteq Q \times \mathcal{P}(\Sigma_X(P)) \times \Gamma(P) \times Q$ is the set of \emph{edges},
% (5) $S \subseteq Q$ is the set of \emph{starting} locations, and (6) $F \subseteq Q$ is the set of \emph{final} locations.
% \end{definition}

